Towards LTE-U Interference Detection, Assessment and Mitigation in 802.11 Networks using Commodity Hardware

We propose WiPLUS -- a system that enables WiFi to deal with the stealthy invasion of LTE-U into the frequency bands used by WiFi. Using solely MAC layer information extracted passively, during runtime, out of the hardware registers of the WiFi NIC at the WiFi access point, WiPLUS is able to: i) detect interfering LTE-U signals, ii) compute their duty-cycles, and iii) derive the effective medium airtime available for each WiFi link in a WiFi Basic Service Set (BSS). Moreover WiPLUS provides accurate timing information about the detected LTE-U ON and OFF phases enabling advanced interference mitigation strategies such as interference-aware scheduling of packet transmissions, rate adaptation and adaptive channel bonding. WiPLUS does not require any modifications to the WiFi client stations and works with commodity WiFi APs where it has a simple software installation process. We present the design, the implementation details and the evaluation of the WiPLUS approach. Evaluation results reveal that it is able to accurately estimate the effective available medium airtime for each link in a WiFi BSS under a wide range of LTE-U signal strengths with a root-mean-square error of less than 3% for the downlink and less 10% for the uplink.

==> packages/config.tex <==
%!TEX root = ../techreport.tex

\usepackage[utf8]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{tabularx}
\usepackage{multicol}
\usepackage{graphicx}

\usepackage{tikz}
\usepackage{lipsum}

\usepackage[headsepline,plainheadsepline,footsepline,plainfootsepline]{scrpage2}


\usepackage{mathptmx}
\usepackage[scaled=.92]{helvet}
\usepackage{courier}

% ================================================================
% FIXME package setup
% ================================================================
\usepackage[multiuser,nomargin,marginclue,footnote]{fixme}
% use different colors for fixme levels
\fxusetheme{color}
\fxsetup{targetlayout=colorcb}
% define authors for fixme
% \FXRegisterAuthor{commnad prefix}{environment prefix}{tag}
\FXRegisterAuthor{awo}{anawo}{AWO}
\FXRegisterAuthor{mc}{anmc}{Mikolaj}
% Usage example \mcfatal{Has to be fixed ASAP}
% Usage example \mcerror{Problem}
% Usage example \mcwarning{Possible problem}
% Usage example \mcnote{Comment}
% fixme mode
% change 'draft' to 'final' for final version
\fxsetup{status=draft}


% ================================================================
% Page Style
% ================================================================

\usepackage{geometry}
\geometry{a4paper, inner=30mm, outer=25mm, top=40mm, bottom=42mm}


\clearscrheadfoot

\ihead[\Large {\scshape TKN Technical Report Series / Technische Universität Berlin }]{\Large {\scshape TU Berlin }}

\ifoot[{\tiny \begin{minipage}{4.0cm}Copyright at Technische Universität Berlin.\newline All Rights reserved.\end{minipage}}]{{\tiny \begin{minipage}{4.0cm}Copyright at Technische Universität Berlin.\newline All Rights reserved.\end{minipage}}}
\cfoot[\scriptsize \trnumber]{\scriptsize \trnumber}
\ofoot[Page \pagemark]{Page \pagemark}

\pagestyle{scrheadings}

\addtokomafont{pagefoot}{\normalfont}



\bibliographystyle{plain}


==> sections/implementation.tex <==
%
% Proposed Approach
%
\section{WiPLUS's Prototype}

\tolja{TODO: move the algorithmic part to design!!!}
As mentioned in the design phase our approach is based on monitoring the state of the WiFi MAC protocol at each AP. For the prototypical implementation we selected WiFi chipsets based on Atheros AR93xx as they allow monitoring of the MAC state machine. 
Fig.~\ref{fig:regmon} illustrates the structure of the signal detection logic of Atheros based WiFi chips. 

The three most interesting building parts such as weak signal detection, strong signal detection and energy detection are depicted.
%Weak signal detection and strong signal detection are independent and complementary features. 

For strong signal detection, it is determined that a signal may exist by the arrival of a stronger signal necessitating a drop in receive gain. This  is  often  referred  to  as  “capture  effect”  in  the
literature. For weak signal detection, it is determined that a signal may exist due to a sudden increase in measured in-band power, followed shortly by a correlation-based algorithm that uses the structue of the preamble signal. Both detectors are triggers to switch the MAC state machine into receive state, while the pure energy detection without strong or weak signal detection pust the MAC into the other busy mode \cite{patent-atheros1}.

%The Weak-signal detection block is used for arriving signals not large enough relative to blockers or noise to cause gain changes. The strong signal detection block is used for larger arriving signals which are determined based upon whether a coarse gain drop or quickdrop gain results.
Moreover, all mentioned MAC states are connected to 32bit registers, which sample the current state using a 40MHz clock. Beside the RX\_BUSY and the  OTHER\_BUSY register, further MAC state registers are available and can be monitored. For our work the following registers are of interest: 
\begin{enumerate}
	\item \textit{TX\_BUSY}: time spent in transmit state,
	\item \textit{RX\_BUSY}: time spent in receive state,
	\item \textit{OTHER\_BUSY}: time spent in energy\_detection state, i.e. energy detected without triggering WiFi packet reception,
	\item \textit{IDLE}: idle time of the MAC.
	\item \textit{ACK\_FAIL}: Number of frames for which no ACK has been received.
\end{enumerate}

%MAC clock rate 40MHZ abtastung 2KHz

\begin{figure}[h!]
\centering
\includegraphics[width=1\linewidth]{figs/atheros_sig_det}
\caption{Block diagram of Atheros signal detection logic and MAC state registers (adapted from~\cite{patent-atheros1}).}
\label{fig:regmon}
\end{figure}

%The LTE-U's share of medium can be calculated 

%Our observation is as follows. As WiFi cannot decode LTE-U frames it has to rely on energy-based carrier sensing. Hence, the LTE-U's share of medium time equals the \textit{OTHER\_BUSY} that correspond to energy detection without triggering packet reception. Observing the \textit{OTHER\_BUSY} is sufficient as long as the LTE-U signal received at the WiFi AP is sufficient strong, i.e. above -62 dBm in case of Atheros chips. Unfortunately, even a weaker LTE-U can distort ongoing WiFi transmissions. In case of Atheros we observed that for weak LTE-U signals \textit{OTHER\_BUSY} is very low and we observed sporadic peaks in the \textit{TX\_BUSY} counter which indicates transmissions attempts being not successful, i.e. not acknowledged. Therefore, in addition we monitor the MAC register counting the number of MAC layer retransmissions, \textit{ACK\_FAIL}. 

The WiPLUS's signal detection component takes as input: i) \textit{OTHER\_BUSY} state and ii) \textit{TX\_BUSY} states suffering from at least one retransmission (\textit{ACK\_FAIL}). The first is used to detect the presence of a strong LTE-U source, i.e. it corresponds to energy detection without triggering packet reception whereas the second is for detection of weak (hidden) LTE-U sources, i.e. indicates transmissions attempts being not successful, i.e. not acknowledged. 
In phase one, cf. Fig.~\ref{fig:wiplus-2step} left, the registers are sampled without any intervention within frame dequeing, while in phase 2, cf. Fig.~\ref{fig:wiplus-2step} middle, the software queues of the ATH9K driver usually used for power saving and frame aggregation, are used to enable a slotted transmission mode, in which every downlink gets a seperate slot assigned, which allows us to monitor every link seperately. For getting access to the registers of the ATH9K MAC FSM and ARQ functionality, we use a modified version of the regmon tool~\cite{Huehn2013} and to enable slotted mode on top of the ATH9k driver we use a modified version of the ATH9k hMAC~\cite{zehl16hmac} tool.

%
%
%
\subsection{Detailed Description}\label{sec:detailed}

A flow chart of WiPLUS describing the steps involved in estimating the LTE-U duty-cycle are depicted in Fig.~\ref{fig:lte-u-flow-chart}:

\begin{figure}[h!]
\centering
\includegraphics[width=0.8\linewidth]{figs/wiplus_pipeline}
\caption{Flow chart of LTE-U duty cycle detector.}
\label{fig:lte-u-flow-chart}
\end{figure}

\textbf{Step 1 -- raw data acquisition:} The input for the first step is data from the Atheros MAC state registers, which we access using the RegMon tool~\cite{Huehn2013}. We sample the MAC state registers with a rate of 2\,kHz (Fig.~\ref{fig:cci_detector_regmon_input}) and process the data in chunks of 1\,s windows size, i.e. $W=2000$ samples:
\begin{align}\label{eq:raw_data_input}
S_t^{\mathrm{TX}}, S_t^{\mathrm{RX}}, S_t^{\mathrm{OTHER}}, S_t^{\mathrm{ACK\_FAIL}}&, \forall t \in 0 \ldots W
\end{align}
where $S_t^{\mathrm{TX}}$, $S_t^{\mathrm{RX}}$ and $S_t^{\mathrm{OTHER}}$ are the relative dwell times for \textit{TX\_BUSY}, \textit{RX\_BUSY} and \textit{OTHER\_BUSY} (e.g. $S_t^{\mathrm{RX}} = 50$ if the MAC stayed 50 percent of the corresponding sample $t$ in the RX state), while $S_t^{\mathrm{ACK\_FAIL}}$ is the number of failed transmissions during sample $t$.

\textbf{Step 2 -- spurious signal extraction:} In the next step we apply signal extraction in which we aim for filtering out noise. For this reason we create a new signal $R_t$:
\begin{align}\label{eq:signal_extraction}
R_t = 
\begin{cases}
    S_t^{\mathrm{OTHER}}, & \text{if } S_t^{\mathrm{TX}}=S_t^{\mathrm{RX}}=0, \\
    S_t^{\mathrm{TX}}, & \text{if } S_t^{\mathrm{ACK\_FAIL}}>0, \\
    S_t^{\mathrm{TX}}, & \forall t': t' \geq t: S_{t'}^{\mathrm{ACK\_FAIL}}>0 \ \wedge \\
    & S_{t \ldots t'}^{\mathrm{TX}} = 100\\
    0, & \text{otherwise}
\end{cases}
\end{align}
While the first case filters out noisy samples, the second and third account for interfered transmission attempts, i.e. unsuccessful transmission due to corruption of either data packet or acknowledgement frame, spanned over single and multiple samples respectively. Note, in \tolja{third we do look-ahead: $R_t$ takes the value of $S_{t}^{\mathrm{TX}}$ if we observe a series of samples with $S_{t}^{\mathrm{TX}} = 100$ followed by an ACK fail.}.

Moreover, we abort the process in case not enough samples could be extracted, $<1\,$\% of samples, i.e. $\frac{\sum_{t \in 1 \ldots W}{\text{sign}(R_t)}}{W} \leq 0.01$.
\michael{C: We abort the process if less than 1\% of the samples in a 1s processing window could be extracted for $R_t$, i.e. if less than 20 out of 2000 samples
could be found that correspond to interfered WiFi transmission. This threshold was found to be feasible during our experiments and
increases the robustness of the algorithm, thus reducing the probability of false detections.}

\textbf{Step 3 -- FFT / PWM signal detection:} In next step we compute the normalized power spectrum of $R_t$ signal using FFT calculation. This is used
as input for a peak detector to find the fundamental frequency, $f_{\mathrm{PWM}_0}$, and second/third harmonics, $f_{\mathrm{PWM}_1}$ and $f_{\mathrm{PWM}_2}$. We abort in case no periodic spectrum can be detected.

\textbf{Step 4 -- clustering:} We use KMeans clustering on $R_t$ to detect cluster centers in time domain. Therefore, we performed clustering for different values for $k = \left\lceil \frac{1}{f_{\mathrm{PWM}_0}} \right\rceil-2 \ldots \left\lceil \frac{1}{f_{\mathrm{PWM}_0}} \right\rceil+2$. We determined the optimal K by silhouette analysis around desired K.
For all $N$ points in a cluster the distance $d_{i,k}$ to the cluster center is calculated, such that $D_{k} = \{d_{i,k} | i=1...N\}$.
\michael{C: Assuming that the points in a cluster are approximately uniformly distributed in time.}
Finally, we set all signal parts outside $2 \times \text{median}(D_{k})$ around cluster centers to zero in order to suppress outliers.

\textbf{Step 5 -- low pass filtering:} We low pass filter the remaining signal to bridge possible gaps, i.e. smoothing.
\michael{C: and to overcome possible imperfections of the KMeans algorithm.}
Therefore, $f_{\mathrm{PWM}_0}$ is used as filter cutoff frequency. We estimate the LTE-U ON time, $T_{\mathrm{ON}}$, by computing median segment duration weighted by energy (area) of the segments (suppress outliers).
\michael{C: We estimate the effective LTE-U ON time, $T_{\mathrm{ON}}$, by computing the mean segment duration of the remaining parts in $R_t > 0$.}

\textbf{Step 5 -- calculate duty cycle:} Finally, we are able to compute the effective LTE-U duty cycle which is: $\mathrm{DutyCylce}_\mathrm{LTE-U} = T_{\mathrm{ON}} \times f_{\mathrm{PWM}_0}$.


\begin{figure}[h!]
\centering
\includegraphics[width=0.85\linewidth]{figs/input_data}
\caption{Input data for WiPLUS: TX (red), RX (blue), Idle (yellow), Other (purple), TX ACK fail (dark red).}
\label{fig:cci_detector_regmon_input}
\end{figure}

% regmon traces: python3 my_regmon_test.py

%\begin{figure}[h!]
%\centering
%\includegraphics[width=1\linewidth]{figs/cci_detector_fir_filtered_signal2}
%\caption{Low pass filtering signal.}
%\label{fig:cci_detector_fir_filtered_signal}
%\end{figure}

%
%
%
\subsection{Discussion}\label{sec:discussion}

\tolja{TODO: Complexity Vergleich von Prototyp mit Implementierung die nur packet capturer nehmen würde. }
